Simplified Continuous High Dimensional Belief Space Planning with Adaptive Probabilistic Belief-dependent Constraints

Online decision making under uncertainty in partially observable domains, also known as Belief Space Planning, is a fundamental problem in robotics and Artificial Intelligence. Due to an abundance of plausible future unravelings, calculating an optimal course of action inflicts an enormous computational burden on the agent. Moreover, in many scenarios, e.g., information gathering, it is required to introduce a belief-dependent constraint. Prompted by this demand, in this paper, we consider a recently introduced probabilistic belief-dependent constrained POMDP. We present a technique to adaptively accept or discard a candidate action sequence with respect to a probabilistic belief-dependent constraint, before expanding a complete set of future observations samples and without any loss in accuracy. Moreover, using our proposed framework, we contribute an adaptive method to find a maximal feasible return (e.g., information gain) in terms of Value at Risk for the candidate action sequence with substantial acceleration. On top of that, we introduce an adaptive simplification technique for a probabilistically constrained setting. Such an approach provably returns an identical-quality solution while dramatically accelerating online decision making. Our universal framework applies to any belief-dependent constrained continuous POMDP with parametric beliefs, as well as nonparametric beliefs represented by particles. In the context of an information-theoretic constraint, our presented framework stochastically quantifies if a cumulative information gain along the planning horizon is sufficiently significant (e.g. for, information gathering, active SLAM). We apply our method to active SLAM, a highly challenging problem of high dimensional Belief Space Planning. Extensive realistic simulations corroborate the superiority of our proposed ideas.

==> floats/means_vars.tex <==
\begin{table} 
	
	\caption{Expected values and variances of (constraining) return given the path within planning session.} 
	
	\centering
	\begin{tabular}{|c|c|c| } 
		
		\hline 
		
		\textnumero path  & $\obj^{(m)}$ & variance $s(b_{k:k+L})$ \\ 
		
		\hline 
		$1 $ & $ -0.0044542 $ & $ 4.67e-5 $ \\ 
		\hline 
		$2 $ & $ -0.0036895 $ & $ 5.25e-5 $ \\ 
		\hline 
		$3 $ & $ -0.0043904 $ & $ 4.59e-5 $ \\ 
		\hline 
		$4 $ & $ -0.003951 $ & $ 4.02e-5 $ \\ 
		\hline 
		$5 $ & $ -0.0032753 $ & $ 4.43e-5 $ \\ 
		\hline 
		$6 $ & $ -0.0019346 $ & $ 7.14e-5 $ \\ 
		\hline 
		$7 $ & $ -0.0021671 $ & $ 6.4e-5 $ \\ 
		\hline 
		$8 $ & $ -0.0016335 $ & $ 7.43e-5 $ \\ 
		\hline 
		$9 $ & $ -0.0015934 $ & $ 7.47e-5 $ \\ 
		\hline 
		$10 $ & $ -0.0016653 $ & $ 9.27e-5 $ \\ 
		\hline 
		$11 $ & $ -0.0033878 $ & $ 5.86e-5 $ \\ 
		\hline 
		$12 $ & $ -0.0028222 $ & $ 5.57e-5 $ \\ 
		\hline 
		$13 $ & $ -0.0030083 $ & $ 7.61e-5 $ \\ 
		\hline 
		$14 $ & $ 0.0009615 $ & $ 5.82e-5 $ \\ 
		\hline 
		$15 $ & $ -0.0039162 $ & $ 4.46e-5 $ \\ 
		\hline 
		$16 $ & $ -0.0004449 $ & $ 6.38e-5 $ \\ 
		\hline 
		$17 $ & $ -0.000847 $ & $ 6.66e-5 $ \\ 
		\hline 
		$18 $ & $ -0.0036301 $ & $ 5.66e-5 $ \\ 
		\hline 
		$19 $ & $ -0.0008257 $ & $ 6.15e-5 $ \\ 
		\hline 
		$20 $ & $ -0.0029662 $ & $ 5.83e-5 $ \\ 
		\hline 
		$21 $ & $ -0.0021627 $ & $ 6.85e-5 $ \\ 
		\hline 
		$22 $ & $ -0.0039177 $ & $ 9.63e-5 $ \\ 
		\hline 
		$23 $ & $ -0.0055105 $ & $ 7.61e-5 $ \\ 
		\hline 
		$24 $ & $ -0.0056228 $ & $ 6.42e-5 $ \\ 
		\hline 
		$25 $ & $ -0.0065283 $ & $ 5.56e-5 $ \\ 
		\hline 
		$26 $ & $ -0.006304 $ & $ 5.96e-5 $ \\ 
		\hline 
		$27 $ & $ -0.0054503 $ & $ 7.06e-5 $ \\ 
		\hline 
		$28 $ & $ -0.0063216 $ & $ 6.37e-5 $ \\ 
		\hline 
		$29 $ & $ -0.0047266 $ & $ 7.84e-5 $ \\ 
		\hline 
		$30 $ & $ -0.005353 $ & $ 6.89e-5 $ \\ 
		\hline 
	\end{tabular} 
\label{tbl:MeanVar} 
\end{table}



